Global Singularity Theory for the Gauss Curvature Equation

Lecture notes for a minicourse to given in the XVII Brazilian School of Geometry, UFAM (Amazonas), Brazil, July 2012.

==> GST_Chap1_150213.tex <==
\catcode`\@=11
\def\triplealign#1{\null\,\vcenter{\openup1\jot \m@th %
\ialign{\strut\hfil$\displaystyle{##}\quad$&\hfil$\displaystyle{{}##}$&$\displaystyle{{}##}$\hfil\crcr#1\crcr}}\,}
\def\multiline#1{\null\,\vcenter{\openup1\jot \m@th %
\ialign{\strut$\displaystyle{##}$\hfil&$\displaystyle{{}##}$\hfil\crcr#1\crcr}}\,}
\catcode`\@=12
%
\newhead{The CNS Method}
%
The Caffarelli-Nirenberg-Spruck (CNS) method yields a-priori second order bounds for smooth solutions of non-linear, hessian-type PDEs given the existence of an upper barrier. It constitutes the main step towards proving the main result of this chapter, namely Theorem \procref{Compactness}, which yields compactness in the $C^\infty$ sense for families of smooth solutions to such PDEs, and, in particular, for families of smooth functions whose graphs have constant gaussian curvature.
\par
The CNS method reduces to a barrier argument (c.f. Chapter $3$ of \cite{GilbTrud}). That is, bounds are obtained by applying the maximum principal to certain, carefully chosen superharmonic functions, which are constructed so as to have suitable properties along the boundary. There is always a certain art to the construction of barrier functions, and the CNS technique is no exception. Consequently, in order to attain a deeper understanding of their approach, we consider it worthwhile to focus on three specific points which we believe stand out. The first is convexity, which is used repeatedly throughout the chapter as a source of positivity. The second is the correct choice of generalised Laplacian with respect to which the superharmonicity of functions will be determined, and which turns out to be the linearisation of the non-linear PDE in question at the function being studied. Finally, the third concerns superharmonicity itself, more precisely, which relations constitute useful upper bounds for intermediate functions and which do not. This is a rather subtle point which will hopefully become clear in Section \subheadref{TheCNSTechnique}, below.
\par
In all situations where the CNS method may be applied, once a-priori second-order bounds have been obtained, higher order bounds follow from general results. First, the Krylov technique (c.f. Theorem \procref{Krylov}) yields a-priori $C^{2+\alpha}$ bounds for solutions. The Schauder technique (c.f. Theorem \procref{Schauder}) then yields a-priori $C^k$ bounds for all $k$, and compactness then follows by the classical Arzela-Ascoli theorem. Since detailed proofs of Theorems \procref{Schauder} and \procref{Krylov} would take us too far afield, we refer the interested reader to \cite{CaffNirSpruckII} and \cite{GilbTrud} for more details.
%
\goodbreak
\newsubhead{The framework}
%
Let $\overline{\Omega}$ be a compact, convex subset of $\Bbb{R}^n$. Let $f\in C^\infty(\overline{\Omega})$ be a smooth, strictly convex function which vanishes along $\partial\Omega$. Let $\kappa:\overline{\Omega}\rightarrow]0,\infty[$ be such that, for all $x$, $\kappa(x)$ is equal to the gaussian curvature of the graph of $f$ at the point $(x,f(x))$. It is a straightforward exercise to show that
\headlabel{TheCNSMethod}
\subheadlabel{TheFramework}
%
$$
\opDet(D^2 f(x)) = \kappa(x)(1 + \|Df(x)\|^2)^{\frac{n+2}{2}}.\eqno{\nexteqnno}
$$
%
We prefer to consider a more general setting which we believe illustrates better the main concepts of the CNS method without introducing excessive complexity. Thus, let $\opSymm:=\opSymm(2,\Bbb{R}^n)$ be the space of real-valued, symmetric matrices of order $n$ and let $\Gamma\subseteq\opSymm$ be the open cone of positive-definite, symmetric matrices. We define the function $F:\Gamma\rightarrow ]0,\infty[$ by
\eqnlabel{GaussCurvatureEquation}
%
$$
F(A) := \opDet(A)^{\frac{1}{n}}.
$$
%
Let $G:\Bbb{R}^n\rightarrow[0,\infty[$ be a smooth, convex function bounded below by $1$. For any smooth function $\phi\in C^\infty(\overline{\Omega},]0,\infty[)$, we now consider smooth, strictly convex functions $f\in C^\infty(\overline{\Omega})$ which satisfy the following non-linear PDE with boundary condition.
%
$$
F(D^2f) = \phi G(Df),\qquad f|_{\partial\Omega} = 0.\eqno{\nexteqnno}
$$
%
We leave the reader to verify that \eqnref{GaussCurvatureEquation} presents a special case of this problem.
\eqnlabel{BasicEquation}
\par
We are interested in studying the problem given the existence of a \gloss{lower barrier}, which is defined to be a smooth, strictly convex function $\hat{f}\in C^\infty(\overline{\Omega})$ which satisfies the following non-linear partial differential inequation with boundary condition.
%
$$
F(D^2\hat{f}) > \phi G(D\hat{f}),\qquad \hat{f}|_{\partial\Omega} = 0.
$$
%
In particular, we define
%
$$
\delta(\hat{f}) := \minf_{x\in\overline{\Omega}}\left(F(D^2\hat{f}(x)) - \phi(x)G(D\hat{f}(x))\right).
$$
%
This quantity will be of use in the sequel.
\par
Given the lower barrier, we are interested in solutions $f$ of \eqnref{BasicEquation} such that $f\geq \hat{f}$. These will be obtained using degree theory, which is a generalisation of the continuity method and will be discussed in Section \headref{HolderSpaces}. This technique requires compactness results for families of solutions of \eqnref{BasicEquation} which are bounded below by corresponding families of lower barriers. Furthermore, by the classical Arzela-Ascoli theorem, such compactness results are equivalent to a-priori bounds for the norms of the $k$'th derivatives of solutions for all $k$. Our main aim is therefore to obtain such bounds. A-priori $C^0$ and $C^1$ bounds follow without further ado.
%
\proclaim{Lemma \nextprocno}
%
\noindent If $f\geq\hat{f}$, then
%
$$\eqalign{
\|f\|_0 &\leq \|\hat{f}\|_0,\cr
\|Df\|_0 &\leq \|D\hat{f}\|_0.\cr}
$$
%
\endproclaim
\proclabel{ZeroethAndFirstOrderBounds}
%
\proof Let $\Delta$ be the standard Laplacian on $\Bbb{R}^n$. Since $f$ is smooth and strictly convex $\Delta f>0$, and so, by the maximum principal,
%
$$
\msup_{x\in\overline{\Omega}}f(x) = \msup_{x\in\partial\Omega}f(x) = 0.
$$
%
Since $f\geq \hat{f}$, it follows that $\|f\|_0\leq\|\hat{f}\|_0$, as desired. We now claim that
%
$$
\|Df\|_0 = \msup_{x\in\partial\Omega}\|Df(x)\|.
$$
%
Indeed, let $x$ be any point of $\Omega$. Denote $V=Df(x)/\|Df(x)\|$ and define $\gamma:\Bbb{R}\rightarrow\Bbb{R}^n$ by $\gamma(t) := x + tV$. Since $\Omega$ is compact and convex, $\gamma^{-1}(\overline{\Omega})$ is a closed interval, $[a,b]$ say, containing $0$. Define $g:[a,b]\rightarrow\Bbb{R}$ by $g(t) := (f\circ\gamma)(t) = f(x + tV)$. Since $f$ is convex, so too is $g$. In particular, $g'$ is monotone, and, without loss of generality we may therefore assume that $g'(b)\geq g'(0) = \|Df(x)\|$. However, using the Cauchy/Schwarz inequality, we obtain
%
$$
\|Df(x)\| \leq g'(b) = \langle Df(\gamma(b)),V\rangle \leq \|Df(\gamma(b))\|\|V\| = \|Df(\gamma(b))\| \leq \msup_{y\in\partial\Omega}\|Df(y)\|,
$$
%
and since $x\in\Omega$ is arbitrary, the assertion follows. However, since $\hat{f}\leq f\leq 0$, and since $\hat{f}=f=0$ along $\partial\Omega$, it follows that, for all $y\in\partial\Omega$,
%
$$
\|Df(y)\| \leq \|D\hat{f}(y)\|,
$$
%
so that $\|Df\|_0\leq\|D\hat{f}\|_0$, as desired. This completes the proof.\qed
\medskip
{\sl\noindent{\bf Remark:\ }The approach described here and in the sequel extends to a far more general framework (c.f. \cite{CaffNirSpruckIII}). Indeed, first let $\opO(n)$ be the group of orthogonal matrices of order $n$, and recall that $\opO(n)$ acts on $\opSymm$ by conjugation. That is, for $M\in\opO(n)$ and for $A\in\opSymm$,
%
$$
M(A) := M^{-1}AM \in\opSymm.
$$
%
Now denote by $\Gamma_0$ the open cone of positive-definite matrices in $\opSymm$, and observe that every element of $\opO(n)$ maps $\Gamma$ bijectively to itself. We then consider any other cone $\Gamma\subseteq\opSymm$ centered on the origen which is convex, invariant under the action of $\opO(n)$ on $\opSymm$, and which, in addition, has the property that for all $x\in\Gamma$, $x + \Gamma_0\subseteq\Gamma$. Given such a $\Gamma$, the theory of Caffarelli, Nirenberg and Spruck applies to a large family of functions $F\in C^\infty(\Gamma)\minter C^0(\overline{\Gamma})$ which are concave, homogeneous of order $1$, invariant under the action of $\opO(n)$ on $\opSymm$, which vanish along the boundary of $\Gamma$, and which satisfy the property that for all $A\in\Gamma$ and for all $B\in\overline{\Gamma}_0\setminus\left\{0\right\}$, $DF(A)(B)>0$.
\par
Although this appears very abstract, we may consider the symmetric polynomials $(\sigma_k)_{0\leq k\leq n}:\opSymm\rightarrow\Bbb{R}$ defined uniquely by the relation
%
$$
\opDet(\opId + tA) =: \sum_{i=0}^nt^i\sigma_i(A),
$$
%
for all $A\in\opSymm$ and for all $t\in\Bbb{R}$. For $0\leq k\leq n$, define $\Gamma_k\subseteq\opSymm$ by
%
$$
\Gamma_k := \left\{ A\ |\ \sigma_0(A),...,\sigma_k(A) > 0\right\},
$$
%
and define $F_k:\Gamma_k\rightarrow[0,\infty[$ by
%
$$
F_k(A):=(\sigma_k(A))^{1/k}.
$$
%
The pair $(\Gamma_k,F_k)$ possesses the properties described above. In particular, when $k=n$, $F_k = \opDet^{1/n}$ and when $k=1$, $F_k=\opTr$, so that the Monge-Amp\`ere operator (studied here) and the Laplacian are in fact both covered by this framework.}
%
\newsubhead{Basic properties of $F$}
%
Higher order a-priori bounds require a deeper understanding of the differential properties of the function $F$. Let $\opEnd(n)$ be the space of linear endomorphisms of $\Bbb{R}^n$. Recall that the canonical inner product of $\opEnd(n)$ can be written in the form
\subheadlabel{BasicPropertiesOfF}
%
$$
\langle A,B\rangle = \opTr(A^tB),
$$
%
and observe that for $A,B\in\opSymm$, this becomes
%
$$
\langle A,B\rangle = \opTr(AB).
$$
%
We identify every linear map $\alpha:\opEnd(n)\rightarrow\Bbb{R}$ with a matrix $A\in\opEnd(n)$ via this inner product. We readily obtain
%
\proclaim{Lemma \nextprocno}
%
\noindent For all $A\in\Gamma$,
%
$$
DF(A) = \frac{1}{n}F(A)A^{-1}.
$$
%
\endproclaim
\proclabel{FirstDerivativeOfF}
%
\noindent In particular, this yields
%
\proclaim{Corollary \nextprocno}
%
\noindent For all $A\in\Gamma$,
%
$$
DF(A)(A) = F(A).
$$
%
\endproclaim
\proclabel{HomogeneityOfF}
%
{\sl\noindent{\bf Remark:\ }This relation in fact follows directly from the homogeneity of $F$.}
%
\proclaim{Lemma \nextprocno}
%
\noindent Suppose that $A\in\Gamma$ is diagonal and let $0<\lambda_1\leq...\leq\lambda_n$ be its eigenvalues. Then, for all $B\in\opSymm$,
%
$$
D^2F(A)(B,B) \leq -\frac{1}{n}F(A)\sum_{i\neq j}\frac{1}{\lambda_i\lambda_j}B_{ij}B_{ij}.
$$
%
\endproclaim
\proclabel{SecondDerivativeOfF}
%
{\sl\noindent{\bf Remark:\ }An analogous relation may be deduced for more general $F$ using the properties of concavity and ellipticity (c.f. \cite{ShengUrbasWang} for details).}
\medskip
\proof Differentiating Lemma \procref{FirstDerivativeOfF} yields
%
$$
D^2F(A)(B,B) = \frac{1}{n}F(A)\left(\frac{1}{n}\opTr(A^{-1}B)^2 - \opTr(A^{-1}BA^{-1}B)\right).
$$
%
Since $A$ is diagonal, this yields
%
$$
D^2F(A)(B,B) = \frac{1}{n}F(A)\left(\frac{1}{n}\sum_{i,j}\frac{1}{\lambda_i\lambda_j}B_{ii}B_{jj} - \sum_{i,j}\frac{1}{\lambda_i\lambda_j}B_{ij}^2\right).
$$
%
However, by the Cauchy/Schwarz inequality,
%
$$
n\sum_{i=1}^n\frac{1}{\lambda_i^2}B_{ii}^2 = \left(\sum_{i=1}^n 1^2\right)\left(\sum_{i=1}^n\frac{1}{\lambda_i^2}B_{ii}^2\right) \geq \left(\sum_{i=1}^n\frac{1}{\lambda_i}B_{ii}\right)^2.
$$
%
The result follows by combining this with the preceeding relation.\qed
\medskip
\noindent In particular, this yields
%
\proclaim{Corollary \nextprocno}
%
\noindent $F$ is concave over $\Gamma$.
%
\endproclaim
\proclabel{ConcavityOfF}
%
We invite the reader to observe the frequency with which the concavity of $F$ and the convexity of $G$ are used throughout the sequel to remove awkward terms. We recall that this is the first key point of the CNS technique. Furthermore, of these two properties, the concavity of $F$ is perhaps more fundamental, as it is used to eliminate third order terms, wheras the convexity of $G$ only eliminates second-order terms.
\medskip
{\sl\noindent{\bf Remark:\ }In particular, in the more general framework described at the end of the previous section, an explicit formula for $DF$ is not necessary. The results obtained in the sequel can be deduced from more general relations derived from the properties of concavity, homogeneity, ellipticity and $\opO(n)$-invariance. See \cite{CaffNirSpruckIII} for details.}
\medskip
Finally, the concavity of $F$ yields the following lower estimate.
%
\proclaim{Lemma \nextprocno}
%
\noindent For all $A$ in $\Gamma$,
%
$$
\frac{1}{n}\opTr(A) \geq F(A).
$$
%
\endproclaim
\proclabel{LowerBoundsOfTraceOfHessian}
%
\proof By concavity,
%
$$
DF(\opId)(A - \opId) \geq F(A) - F(\opId).
$$
%
Thus, using Lemma \procref{FirstDerivativeOfF} and the fact that $F(\opId)=1$, we obtain
%
$$\triplealign{
&\frac{1}{n}\opTr(A-\opId)&\geq F(A) - 1\cr
\Rightarrow&\frac{1}{n}\opTr(A)&\geq F(A),\cr}
$$
%
as desired.\qed
%
\newsubhead{Linearisation}
%
We obtain estimates using the maximum principle, and for this reason superharmonic functions will play an important role in what follows. Importantly, however, the concept of ``superharmonicity'' depends implicitely on the choice of generalised Laplacian used, and the correct choice constitutes the second key point of the CNS technique. We thus define $\Cal{L}_f:C^\infty(\overline{\Omega})\rightarrow C^\infty(\overline{\Omega})$ by
\subheadlabel{Linearisation}
%
$$
\Cal{L}_f g := DF(D^2f)(D^2g) - \phi DG(Df)(Dg).
$$
%
The informed reader will notice that this is precisely the linearisation at $f$ of the partial differential operator $\Phi$ given by $\Phi(Dg,D^2g) = F(D^2g) - \phi G(Dg)$ (c.f. Section \headref{HolderSpaces}).
%
\proclaim{Lemma \nextprocno}
%
\noindent $\Cal{L}_f$ is a second-order, linear, elliptic, partial differential operator.
%
\endproclaim
\proclabel{Ellipticity}
%
\proof By definition, $\Cal{L}_f$ is a second-order, linear, partial differential operator. It thus remains to show ellipticity. Let $\sigma_2(\Cal{L}_f)$ be the principle symbol of $\Cal{L}_f$ (c.f. \cite{FriedlanderJoshi}). We have to show that $\sigma_2(\Cal{L}_f)$ is everywhere positive definite. Using Lemma \procref{FirstDerivativeOfF}, we obtain
%
$$\eqalign{
\sigma_2(\Cal{L}_f)(\xi) &= DF(D^2f)(\xi\otimes\xi)\cr
&= \frac{1}{n}F(D^2f)\opTr((D^2f)^{-1}(\xi\otimes\xi))\cr
&= \frac{1}{n}F(D^2f)\langle\xi, (D^2f)^{-1}\xi\rangle.\cr}
$$
%
However, since $f$ is strictly convex, $D^2f$ is positive definite at every point, and therefore so too is its inverse. The principle symbol of $\Cal{L}_f$ is thus also everywhere positive definite, as desired.\qed
\medskip
The following result provides an important source of superharmonic functions to be used in the sequel.
%
\proclaim{Theorem \nextprocno}
%
\noindent If $\delta\geq 0$ is a non-negative real number and if $g,h\in C^\infty(\overline{\Omega})$ are smooth, strictly convex functions such that
%
$$
F(D^2g) = \phi G(Dg),\qquad F(D^2h) \geq \phi G(Dh) + \delta,
$$
%
then
%
$$
\Cal{L}_g(g-h) \leq -\delta.
$$
%
\endproclaim
\proclabel{SuperHarmonicFunctions}
%
\proof By definition,
%
$$
F(D^2g) - \phi G(Dg) = 0 \leq F(D^2h) - \phi G(Dh) - \delta.
$$
%
By concavity of $F$,
%
$$
DF(D^2g)(D^2g - D^2h) \leq F(D^2g) - F(D^2h).
$$
%
By positivity of $\phi$ and convexity of $G$,
%
$$
\phi DG(Dg)(Dh - Dg) \leq \phi G(Dh) - \phi G(Dg).
$$
%
Combining the above relations and recalling the definition of $\Cal{L}_g$ yields
%
$$
\Cal{L}_g(g - h) \leq -\delta,
$$
%
as desired.\qed
\medskip
\noindent This yields in particular the strong maximum principal in the non-linear setting.
%
\proclaim{Lemma \nextprocno}
%
\noindent Let $g,h\in C^\infty(\Omega)$ be strictly convex functions such that $F(D^2h)/G(Dh) \geq F(D^2g)/G(Dg)$ and let $p$ be a point in $\overline{\Omega}$ where $g-h$ attains its minimum value. If $D(g-h)=0$ at $p$, then $(g-h)$ is constant.
%
\endproclaim
\proclabel{StrongMaximumPrinciple}
%
{\sl\noindent{\bf Remark:\ }In particular, if $p$ is an interior point, then $D(g-h)=0$ at $p$, so that if $(g-h)$ attains its minimum value at any interior point, then it is constant. This is the usual formulation of the strong maximum principal.}
\medskip
\proof Suppose the contrary, so that $g-h$ is non-constant. Define the function $\psi$ by $\psi := F(D^2g)/G(Dg)>0$. In particular,
%
$$
F(D^2h) - \psi G(Dh) \geq 0 =  F(D^2g) - \psi G(Dg).
$$
%
Thus, by Theorem \procref{SuperHarmonicFunctions} applied with $\phi=\psi$,
%
$$
\Cal{L}_g(g - h) \leq 0.
$$
%
It follows from Hopf's maximum principle (c.f. Lemma $3.4$ of \cite{GilbTrud}) that $D(g-h)\neq 0$ at $p$. This is absurd by hypothesis, and we conclude that $g-h$ is constant, as desired.\qed
%
\newsubhead{The CNS technique}
%
Let $X$ be a smooth vector field in $\Bbb{R}^n$ tangent to $\partial\Omega$. In particular, and importantly, the function $Xf=Df(X)$ vanishes along the boundary. It is this function that we aim to control using the maximum principal. To this end, we first obtain a-priori bounds for $\Cal{L}_f(Xf)$. Importantly, although absolute bounds do not exist, $\Cal{L}_f(Xf)$ is controlled by a certain function which depends on the data. This is the third key point of the CNS technique: understanding that the terms that are really useful are precisely those that are bounded by this function. We thus define
\subheadlabel{TheCNSTechnique}
%
$$
B^{ij} = \frac{1}{n}F(D^2f)(D^2f^{-1})^{ij},
$$
%
so that $B$ is the matrix of $DF(D^2f)$, and we define
%
$$
\Lambda(f) := DF(D^2f)(\opId) = B^{ij}\delta_{ij}.
$$
%
Fixed multiples of $\Lambda(f)$ also bound terms that are already known to be bounded by constants. Indeed, we have
%
\proclaim{Lemma \nextprocno}
%
\noindent For all $f$,
%
$$
\Lambda(f)\geq 1.
$$
%
\endproclaim
\proclabel{LambdaIsGreaterThanOne}
%
{\sl\noindent{\bf Remark:\ }Observe that the proof is valid for any concave $F$ homogeneous of order $1$ such that $F(\opId)=1$ (c.f. the remark following Corollary \procref{HomogeneityOfF}).}
\medskip
\proof Indeed, by Corollary \procref{HomogeneityOfF}, for all $A\in\Gamma$,
%
$$
DF(A)(A) = F(A).
$$
%
However, since $F$ is concave,
%
$$
DF(A)(\opId - A) \geq F(\opId) - F(A) = 1 - F(A).
$$
%
Thus, by linearity,
%
$$\eqalign{\opTr(DF(A))&=DF(A)(\opId)\cr
&=DF(A)(\opId - A) + DF(A)(A)\cr
&\geq 1 - F(A) + F(A)\cr
&= 1,\cr}$$
%
as desired.\qed
\medskip
We now control $\Cal{L}_f(Xf)$.
%
\proclaim{Lemma \nextprocno}
%
\noindent There exists $C>0$ which only depends on $\|\phi\|_1$, $\|X\|_2$ and $\|f\|_1$ such that,
%
$$
\left|\Cal{L}_f(Xf)\right| \leq C\Lambda(f).
$$
%
\endproclaim
\proclabel{OffNormalDerivatives}
%
{\sl\noindent{\bf Remark:\ }Observe that the proof only uses the homogeneity of $F$. Indeed, the idea is that since $f$ is a solution of \eqnref{BasicEquation}, any derivative of $f$ should satisfy the linearisation of \eqnref{BasicEquation} (c.f. Section \headref{HolderSpaces}) modulo lower order terms. However, there is a problem, since $\Cal{L}_f(Xf)$ actually involves terms which are of second-order in $f$. Nonetheless, these are readily removed using Corollary \procref{HomogeneityOfF}, which, as remarked previously, only really requires the homogeneity of $F$.}
\medskip
\proof For all $i$, differentiate \eqnref{BasicEquation} in the direction of $e_i$. Since $D^3f$ is symmetric, by definition of $\Cal{L}_f$, for all $i$, this yields
%
$$
\Cal{L}_f f_i = \phi_i G(Df).
$$
%
Thus, using the summation convention,
%
$$
X^i\Cal{L}_ff_i = X^i\phi_i G(Df).
$$
%
There therefore exists $C_1>0$ which only depends on $\|\phi\|_1$ and $\|f\|_1$ such that
%
$$
\left| X^i\Cal{L}_f f_i\right| \leq C_1.
$$
%
We aim to move $X^i$ to the other side of $\Cal{L}_f$. To this end, we define the operator $\Cal{L}^1_f$ by
%
$$
\Cal{L}^1_f g := -\phi DG(Df)(Dg).
$$
%
That is, $\Cal{L}^1_f$ is the first order component of $\Cal{L}_f$. By the chain rule,
%
$$
\Cal{L}^1_f(X^i f_i) - X^i\Cal{L}^1_f(f_i) = f_i\Cal{L}^1_f(X^i).
$$
%
There therefore exists $C_2>0$ which only depends on $\|\phi\|_0$, $\|f\|_1$ and $\|X\|_1$ such that,
%
$$
\left|\Cal{L}^1_f(X^if_i) - X^i\Cal{L}^1_f(f_i)\right| \leq C_2.
$$
%
Furthermore, by Lemma \procref{SecondDerivativeOfF},
%
$$\multiline{
X^iDF(D^2f)(D^2f_i) - DF(D^2f)(D^2(Xf))& \cr
\qquad\qquad= X^iB^{pq}f_{ipq} - B^{pq}(X^if_i)_{pq}& \cr
\qquad\qquad= - B^{pq}{X^i}_pf_{iq} - B^{pq}{X^i}_qf_{ip} - B^{pq}{X^i}_{pq}f_i.& \cr}$$
%
However, using the fact that $f$ is a solution of \eqnref{BasicEquation}, we obtain
%
$$
B^{pq}f_{ip} = \frac{1}{n}F(D^2f){\delta^q}_i = \frac{1}{n}\phi G(Df){\delta^q}_i.
$$
%
This eliminates the terms on the right hand side which are of second-order in $f$. We remark in passing that this is the step in which the homogeneity of $F$ is required. We conclude that there exists $C_3>0$, which only depends on $\|\phi\|_0$, $\|X\|_2$ and $\|f\|_1$ such that
%
$$
\left|X^iDF(D^2f)(D^2f_i) - DF(D^2f)(D^2(Xf))\right| \leq C_3\Lambda(f).
$$
%
Combining the above relations, and using Lemma \procref{LambdaIsGreaterThanOne} along with the triangle inequality, we obtain
%
$$\eqalign{
\left|\Cal{L}_f(Xf)\right| &\leq \left|DF(D^2f)(D^2(Xf)) - X^iDF(D^2f)(D^2f_i)\right|\cr
&\qquad +\left|\Cal{L}^1_f(X^if_i) - X^i\Cal{L}^1_f(f_i)\right| + \left|X^i(\Cal{L}_ff_i)\right|\cr
&\leq C_1 + C_2 + C_3\Lambda(f)\cr
&\leq (C_1 + C_2 + C_3)\Lambda(f),\cr}$$
%
as required.\qed
\medskip
We now introduce the first component of the barrier function which the CNS technique uses to provide a-priori bounds for $Xf$. Consider the function $f-\hat{f}$. This function is non-negative, and by Theorem \procref{SuperHarmonicFunctions}, is superharmonic with respect to $\Cal{L}_f$. We now perturb it to be strictly negative away from a given boundary point whilst maintaining superharmonicity. Thus, for all $p\in\partial\Omega$, and for all $\epsilon>0$, we define
%
$$
\hat{f}_{p,\epsilon}(x) := \hat{f}(x) - \epsilon\|x-p\|^2.
$$
%
\proclaim{Lemma \nextprocno}
%
\noindent There exists $\epsilon_0>0$, which only depends on $\|\phi\|_0$, $\delta(\hat{f})$ and $\|\hat{f}\|_2$ such that, for all $p\in\partial\Omega$, and for all $\epsilon<\epsilon_0$,
%
$$
\Cal{L}_f(f - \hat{f}_{p,\epsilon}) \leq 0.
$$
%
\endproclaim
\proclabel{FirstBarrierFunction}
%
\proof Indeed, by compactness, there exists $\epsilon_0>0$ which only depends on $\|\phi\|_0$, $\delta(\hat{f})$ and $\|\hat{f}\|_2$ such that for all $p\in\partial\Omega$ and for all $\epsilon<\epsilon_0$,
%
$$
F(D^2\hat{f}_{p,\epsilon}) \geq \phi G(D\hat{f}_{p,\epsilon}).
$$
%
The result now follows by Theorem \procref{SuperHarmonicFunctions}.\qed
\medskip
For all $p\in\partial\Omega$, we define the function $d_p:\Omega\rightarrow\Bbb{R}$ by
%
$$
d_p(x) := \|x - p\|.
$$
%
This is the second component of the CNS barrier function.
%
\proclaim{Lemma \nextprocno}
%
\noindent There exists $r>0$, which only depends on $\|\phi\|_0$ and $\|f\|_1$ such that, for all $p\in\partial\Omega$,
%
$$
\Cal{L}_f d_p^2 \geq \Lambda(f),
$$
%
over $\Omega\minter B_r(p)$.
%
\endproclaim
\proclabel{SecondBarrierFunction}
%
\proof By definition, for all $g$,
%
$$
\Cal{L}_f g = DF(D^2f)(D^2g) - \phi DG(Df)(Dg).
$$
%
However, when $g=d_p^2$, for all $x$,
%
$$
\|Dg(x)\| = 2d_p(x).
$$
%
Thus, bearing in mind Lemma \procref{LambdaIsGreaterThanOne}, there exists $r>0$ which only depends on $\|\phi\|_0$ and $\|f\|_1$ such that, for $d_p(x)<r$,
%
$$
\left|\phi(x)DG(Df(x))(Dg(x))\right| \leq 1 \leq \Lambda(f)(x).
$$
%
However, for all $x$,
%
$$
DF(D^2f(x))(D^2d_p^2(x)) = DF(D^2f(x))(2\opId) = 2\Lambda(f)(x).
$$
%
The result now follows by subtracting these two relations.\qed
\medskip
The following result lies at the heart of the CNS technique.
%
\proclaim{Lemma \nextprocno}
%
\noindent There exists $C>0$, which only depends on $\|\phi\|_1$, $\|X\|_2$, $\delta(\hat{f})$, $\|\hat{f}\|_2$ and $\|f\|_1$ such that if $f\geq \hat{f}$, then for all $p\in\partial\Omega$,
%
$$
\|D(Xf)(p)\| \leq C.
$$
%
\endproclaim
\proclabel{OffNormalSecondOrderBounds}
%
\proof Let $C$ be as in Lemma \procref{OffNormalDerivatives} and let $r$ be as in Lemma \procref{SecondBarrierFunction}. For all $p\in\partial\Omega$, throughout $\Omega\minter B_r(p)$,
%
$$
-\Cal{L}_f(Cd_p^2) \leq \Cal{L}_f(Xf) \leq \Cal{L}_f(Cd_p^2).
$$
%
Now let $\epsilon<\epsilon_0$ be as in Lemma \procref{FirstBarrierFunction}. For all $A>0$, and for all $p\in\partial\Omega$, throughout $\Omega\minter B_r(p)$,
%
$$
\Cal{L}_f(A(f-\hat{f}_{p,\epsilon}) - Cd_p^2) \leq \Cal{L}_f(Xf) \leq \Cal{L}_f(-A(f - \hat{f}_{p,\epsilon}) + Cd_p^2).
$$
%
For $p\in\partial\Omega$, $\partial (\Omega\minter B_r(p))$ consists of two components, namely $B_r(p)\minter\partial\Omega$ and $\Omega\minter \partial B_r(p)$. Furthermore, for all $p\in\partial\Omega$,
%
$$
f - \hat{f}_{p,\epsilon} \geq \epsilon d_p^2.
$$
%
Setting $A>C\epsilon^{-1} + \|X\|_0\|f\|_1\epsilon^{-1}r^{-2}$, we obtain, for all $p\in\partial\Omega$, and for all $x\in\partial\Omega$,
%
$$
(A(f - \hat{f}_{p,\epsilon}) - Cd_p^2)(x) \geq 0=\left|(Xf)(x)\right|.
$$
%
Likewise, for all $p\in\partial\Omega$, and for all $x\in\Omega\minter\partial B_r(p)$,
%
$$
(A(f - \hat{f}_{p,\epsilon}) - Cd_p^2)(x) \geq \left|(Xf)(x)\right|.
$$
%
That is, for all $p\in\partial\Omega$, and for all $x\in\partial(\Omega\minter B_r(p))$,
%
$$
(A(f - \hat{f}_{p,\epsilon_0}) - Cd_p^2)(x) \geq (Xf)(x) \geq -(A(f - \hat{f}_{p,\epsilon_0}) - Cd_p^2)(x).
$$
%
We conclude by the maximum principle that for all $p\in\partial\Omega$,
%
$$
A(f - \hat{f}_{p,\epsilon_0}) - Cd_p^2 \geq Xf \geq -A(f - \hat{f}_{p,\epsilon_0}) + Cd_p^2
$$
%
throughout $\Omega\minter B_r(p)$. However, by definition, these three functions are all equal to $0$ at $p$, so that
%
$$\eqalign{
\|D(Xf)(p)\| &\leq A\|D(f - \hat{f}_{p,\epsilon_0})(p)\|\cr
&= A\|D(f-\hat{f})(p)\|\cr
&\leq A(\|f\|_{C^1} + \|\hat{f}\|_{C^1}),\cr}$$
%
as desired.\qed
\medskip
Now fix $p\in\partial\Omega$. Upon applying an isometry of $\Bbb{R}^n$, we may suppose that $p=0$ and that the tangent space to $\partial\Omega$ at $p$ is spanned by the vectors $e_1,...,e_{n-1}$. For all $r$, let $B'_r(0)$ be the ball of radius $r$ about $0$ in $\Bbb{R}^{n-1}$. For sufficiently small $r$, there exists a smooth function $\omega:B'_r(0)\rightarrow]-r,r[$ whose graph coincides with $\partial\Omega\minter (B_r'(0)\times]-r,r[)$. Using this construction, Lemma \procref{OffNormalSecondOrderBounds} is now expressed as follows.
%
\proclaim{Corollary \nextprocno}
%
\noindent There exists $C>0$ which only depends on $\|\phi\|_1$, $\delta(\hat{f})$, $\|\hat{f}\|_2$ and $\|f\|_1$ such that if $f\geq\hat{f}$ then, for all $(i,j)\neq(n,n)$,
%
$$
\left|f_{ij}(0)\right| \leq C.
$$
%
\endproclaim
\proclabel{CorOffNormalSecondOrderBounds}
%
\proof Since $D^2f$ is symmetric, we may suppose that $j<n$. Let $\chi\in C_0^\infty(B'_r(0)\times]-r,r[)$ be a smooth function of compact support equal to $1$ near $0$, and define the vector field $X_j$ by
%
$$
X_j(x',t) := \chi(x',t)(e_j,\omega_j(x')).
$$
%
Observe that $X_j$ is tangent to $\partial\Omega$ and that $\|X_j\|_2$ is controlled by the geometry of $\Omega$. Moreover, $(D\omega)(0)=0$ and so $X_j(0,0) = e_j$. Thus, for all $1\leq i\leq n$,
%
$$
\left|f_{ij}(0)\right| \leq \|D(X_jf)(0)\| + \left|f(0)(\partial_i X_j)(0)\right|,
$$
%
and the result now follows by Lemma \procref{OffNormalSecondOrderBounds}.\qed
%
\newsubhead{The double normal derivative}
%
By Corollary \procref{CorOffNormalSecondOrderBounds}, it only remains to control the second derivative in the double normal direction. In more general applications of the CNS technique, this actually presents a serious difficulty, often requiring a further, lengthy barrier argument (c.f. \cite{CaffNirSpruckII}). However, in the current case, this term is controlled by a straightforward ad-hoc argument which we now describe. We continue to use the notation introduced at the end of Section \subheadref{TheCNSTechnique}, and we thus aim to control $\left|f_{nn}(0)\right|$.
%
\proclaim{Lemma \nextprocno}
%
\noindent For all $B>0$, there exists $C>0$ with the property that if $M$ is a symmetric $n\times n$ matrix such that
\medskip
\myitem{(1)} $\left|M_{ij}\right|<B$ for all $(i,j)\neq (n,n)$;
\medskip
\myitem{(2)} $\left|\opDet(M)\right|<B^n$; and
\medskip
\myitem{(3)} $\left|\opDet(M')\right|>B^{-1}$,
\medskip
\noindent where $M'$ is the $(n-1)\times(n-1)$ matrix given by the upper-left hand corner of $M$, then,
%
$$
\left|M_{nn}\right| \leq C.
$$
%
\endproclaim
\proclabel{FinalStep}
%
\proof Indeed, by hypothesis,
%
$$
B^n > \left|\opDet(M)\right| > \left|M_{nn}\right|\left|\opDet(M')\right| - (n-1)(n-1)!B^n,
$$
%
and the result follows with $C:=(1 + (n-1)(n-1)!)B^{n+1}$.\qed
\medskip
\noindent It thus suffices to obtain lower bounds for the absolute value of the determinant of $(f_{ij}(0))_{1\leq i,j\leq (n-1)}$.
%
\proclaim{Lemma \nextprocno}
%
\noindent For all $\epsilon>0$, there exists $\delta>0$, which only depends on $\epsilon$ and the geometry of $\Omega$ such that if $f_n(0)<-\epsilon$, then
%
$$
\left|\opDet((f_{ij}(0))_{1\leq i,j\leq (n-1)})\right| > \delta.
$$
%
\endproclaim
\proclabel{OffNormalSecondOrderLowerBounds}
%
\proof By definition, $D\omega(0)=0$ and since $\Omega$ is strictly convex, so too is $\omega$. Now observe that the function $x'\mapsto f(x',\omega(x'))$ vanishes identically. Thus, by the chain rule, for all $1\leq i,j\leq (n-1)$,
%
$$
f_{ij} + f_n\omega_{ij} = 0.
$$
%
In particular, by definition of $\epsilon$,
%
$$
\left|\opDet((f_{ij}(0))_{1\leq i,j\leq (n-1)})\right| > \epsilon^{n-1}\left|\opDet(\omega_{ij}(0))\right|,
$$
%
and the result follows.\qed
\medskip
\noindent We now bound $f_n$ from above via an ad-hoc barrier argument.
%
\proclaim{Lemma \nextprocno}
%
\noindent There exists $\delta>0$ which only depends on $\minf_{x\in\overline{\Omega}}\phi(x)$ such that $f_n(p)<-\delta$.
%
\endproclaim
\proclabel{FirstOrderLowerBounds}
%
\proof We continue to consider $\Bbb{R}^n$ as the product $\Bbb{R}^{n-1}\times\Bbb{R}$. Since $\partial\Omega$ is smooth, there exists $r>0$, which only depends on the geometry of $\Omega$, such that $B_r((0,r))$ is contained within $\Omega$. For all $\delta>0$, define $h_{\delta}\in C^\infty(B_r((0,r)))$ by
%
$$
h_\delta(x) := \delta \| x - (0,r) \| ^ 2 - \delta r^2.
$$
%
Observe that $F(D^2h_\delta)=2\delta$ and so, for $2\delta<\minf_{x\in\overline{\Omega}}\phi(x)$,
%
$$
F(D^2h_\delta) - \phi G(Dh_\delta)\leq 0 = F(D^2f) - \phi G(Df).
$$
%
However, for all $x\in\partial B_r((0,r))$,
%
$$
(h_\delta - f)(x) = -f(x) \geq 0.
$$
%
It thus follows by the maximum principal (Lemma \procref{StrongMaximumPrinciple}) that $h_\delta - f\geq 0$ throughout $B_r((0,r))$. Since $h_\delta$ and $f$ coincide at $0$, this yields
%
$$
f_n(0) \leq (\partial_n h_\delta)(0) = -2\delta r,
$$
%
as desired.\qed
\medskip
\noindent We thus obtain a-priori second order bounds for $f$ at every boundary point of $\Omega$.
%
\proclaim{Theorem \nextprocno}
%
\noindent There exists $C>0$ which only depends on $\|\phi\|_1$, $\minf_{x\in\overline{\Omega}}\phi(x)$, $\delta(\hat{f})$, $\|\hat{f}\|_2$ and $\|f\|_1$ such that if $f\geq\hat{f}$ then, for all $x\in\partial\Omega$,
%
$$
\|D^2 f(x)\| \leq C.
$$
%
\endproclaim
\proclabel{SecondOrderBounds}
%
\proof By Corollary \procref{CorOffNormalSecondOrderBounds}, there exists $C_1>0$ which only depends on $\|\phi\|_1$, $\delta(\hat{f})$, $\|\hat{f}\|_2$ and $\|f\|_1$ such that if $f\geq\hat{f}$ then, for all $(i,j)\neq (n,n)$,
%
$$
\left|f_{ij}(0)\right| \leq C_1.
$$
%
By Lemma \procref{FirstOrderLowerBounds}, there exists $\delta_1>0$ such that
%
$$
f_n(0) \leq -\delta_1.
$$
%
By Lemma \procref{OffNormalSecondOrderLowerBounds} there exists $\delta_2>0$, which only depends on $\delta_1$ and $C_1$ such that
%
$$
\left|\opDet((f_{ij}(0))_{1\leq i,j\leq (n-1)})\right| \geq \delta_2.
$$
%
Thus, by Lemma \procref{FinalStep}, there exists $C_2>C_1$, which only depends on $\delta_2$ and $C_1$, such that
%
$$
\left|f_{nn}(0)\right| \leq C_2,
$$
%
and we conclude that $\|Df(0)\|\leq C_2$, as desired.\qed
%
\newsubhead{Boundary to global}
%
We have obtained a-priori second-order bounds for $f$ for every boundary point of $\Omega$, and we now use the maximum principal to extend these to global second-order bounds over the whole of $\Omega$. Since the problem is non-linear, this is not wholly trivial, and the technique that we use relies on the existence of a superharmonic auxiliary function. In the present case, we use the function $f-\hat{f}$, which is always defined over the whole of $\Omega$. However, in more general settings, suitable auxiliary functions do not always exist, so that this becomes another criteria in determining whether or not the Plateau problem has a solution over over a given domain.
\subheadlabel{BoundaryToGlobal}
\par
Let $\lambda_1,...,\lambda_n:\Omega\rightarrow\Bbb{R}$ be such that, for all $x$, $0<\lambda_1(x)\leq...\leq\lambda_n(x)$ are the eigenvalues of $D^2f(x)$, and, for all $1\leq i\leq n$, define $\mu_i:\Omega\rightarrow\Bbb{R}$ by $\mu_i:=\opLog(\lambda_i)$. Observe that although these functions are continuous, they are not necessarily smooth. It is therefore useful to introduce the following definition.
%
\proclaim{Definition \nextprocno}
%
\noindent Let $U\subseteq\Bbb{R}^n$ be an open set, let $L$ be a second-order, linear, partial differential operator defined over $U$, let $f:U\rightarrow\Bbb{R}$ be a continuous function and let $g:U\times\Bbb{R}^n\rightarrow\Bbb{R}$ be any other function. We say that $(Lf)(x)>g(x,Df(x))$ in the weak sense whenever, for all $x\in U$, there exists a smooth function $\alpha$ such that
\medskip
\myitem{(1)} $\alpha(x)=f(x)$;
\medskip
\myitem{(2)} $\alpha\leq f$; and
\medskip
\myitem{(3)} $(L\alpha)(x)>g(x,D\alpha(x))$.
%
\endproclaim
\proclabel{DefinitionWeakSolutions}
%
{\sl\noindent{\bf Remark:\ }The informed reader will notice similarities with the concept of viscosity supersolutions (c.f. \cite{CrandhallIshiiLyons}). Definition \procref{DefinitionWeakSolutions} however yields a stronger property, since the definition of viscosity solutions does not require the existence of smooth test functions at every point.}
\medskip
\noindent We now recall the matrix $B^{ij}$ defined in Section \subheadref{TheCNSTechnique}.
%
\proclaim{Lemma \nextprocno}
%
\noindent If $g:\overline{\Omega}\rightarrow\Bbb{R}$ is a smooth, positive function, then
%
$$
\Cal{L}_f \opLog(g) = \frac{1}{g}\Cal{L}_f g - B^{ij}\partial_i\opLog(g)\partial_j\opLog(g).
$$
%
\endproclaim
\proclabel{DerivativeOfLogarithm}
%
\proof Indeed, by the chain rule,
%
$$\eqalign{
D\opLog(g) &= \frac{1}{g}Dg,\cr
(D^2\opLog(g))_{ij} &= \frac{1}{g}(D^2g)_{ij} - (D\opLog(g))_i(D\opLog(g))_j.\cr}
$$
%
Since $DF(D^2f)$ and $DG(Df)$ are linear, this yields
%
$$\eqalign{
\Cal{L}_f\opLog(g) &= DF(D^2f)(D^2\opLog(g)) - \phi DG(Df)(D\opLog(g))\cr
&= \frac{1}{g}DF(D^2f)(D^2g) - \frac{1}{g}\phi DG(Df)(Dg) - DF(D^2f)^{ij}(D\opLog(g))_i(D\opLog(g))_j\cr
&= \frac{1}{g}\Cal{L}_fg - DF(D^2f)^{ij}(D\opLog(g))_i(D\opLog(g))_j,\cr}$$
%
as desired.\qed
%
\proclaim{Lemma \nextprocno}
%
\noindent There exists $C>0$, which only depends on $\|\phi\|_2$, $\|f\|_1$ and $\minf_{x\in\overline{\Omega}}\phi(x)$ such that if $x\in\overline{\Omega}$ and if $e_n$ coincides with the eigenvector of $D^2f(x)$ corresponding to the greatest eigenvalue $\lambda_n$, then, at $x$,
%
$$
\Cal{L}_f\mu_n + \frac{2}{n\lambda_n}(\partial_n\mu_n)^2 \geq -C + B^{ij}(\partial_i\mu_n)(\partial_j\mu_n)
$$
%
in the weak sense.
%
\endproclaim
\proclabel{ThirdBarrierFunction}
%
{\sl\noindent{\bf Remark:\ }Observe that the coefficient of the second term on the left-hand side tends to zero as $\lambda_n$ tends to infinity. Furthermore,  although the coefficient of the second term on the right-hand side of in Lemma \procref{DerivativeOfLogarithm} is negative, the coefficient of the corresponding term in the above formula is positive. Since this latter is a consequence of Lemma \procref{SecondDerivativeOfF}, it continues to hold for more general functions $F$ which are convex and elliptic. Both these properties will play an important role in the sequel.}
\medskip
\proof Choose $x\in\Omega$. By applying an isometry, we may assume that $e_1,...,e_n$ are the eigenvectors of $D^2f(x)$ corresponding to the eigenvalues $\lambda_1(f)(x),...,\lambda_n(f)(x)$ respectively. Define $\alpha(x):=\opLog(f_{nn}(x))$. Observe that $\alpha$ is smooth, $\alpha\leq\mu_n(f)$ and $\alpha(x)=\mu_n(f)(x)$. It thus suffices to prove the desired relation for $\alpha$ at $x$. Differentiating \eqnref{BasicEquation} twice in the $e_n$ direction at $x$ yields
%
$$\multiline{
DF(D^2f(x))(\partial_n\partial_n D^2f(x)) + D^2F(D^2f(x))(\partial_n D^2 f(x),\partial_n D^2 f(x))& \cr
\qquad = \phi_{nn}(x)G(Df(x)) + 2\phi_n(x)DG(Df(x))(\partial_n Df(x))& \cr
\qquad\qquad  + \phi(x)DG(Df(x))(\partial_n\partial_n Df(x)) + \phi(x)D^2g(Df(x))(\partial_n Df(x),\partial_n Df(x)).& \cr}
$$
%
Since the derivatives of $f$ are symmetric, since $G$ is convex, since $\phi$ is positive and recalling the definition of $\Cal{L}_f$, this simplifies to
%
$$\eqalign{
(\Cal{L}_f f_{nn})(x) &\geq \phi_{nn}(x)G(Df(x)) + 2\phi_n(x)DG(Df(x))(Df_n(x))\cr
&\qquad - D^2F(D^2f(x))(D^2 f_n(x),D^2 f_n(x)).\cr}
$$
%
Since $\|D^2f(x)\|\leq\lambda_n(x)=f_{nn}(x)$, there exists $C_1>0$ which only depends on $\|\phi\|_2$ and $\|f\|_1$ such that
%
$$
(\Cal{L}_f f_{nn})(x) \geq -C_1-C_1\lambda_n(x)-D^2F(D^2f(x))(D^2 f_n(x),D^2 f_n(x)).
$$
%
However, by Lemma \procref{SecondDerivativeOfF} and the positivity of $D^2f(x)$,
%
$$\multiline{
-(D^2F)(D^2f(x))(D^2 f_n(x),D^2 f_n(x))\geq \frac{1}{n}F(D^2f(x))\sum_{i\neq j}\frac{1}{\lambda_i(x)\lambda_j(x)}(f_{ijn})(x)^2& \cr
\qquad\qquad\geq \frac{2}{n}F(D^2f(x))\lambda_n(x)\sum_{i=1}^{n-1}\frac{1}{\lambda_i(x)\lambda_n^2(x)}(f_{inn})(x)^2& \cr
\qquad\qquad= 2\lambda_n(x)B^{ij}(\partial_i\opLog(f_{nn})(x))(\partial_j\opLog(f_{nn})(x)) - \frac{2}{n}(\partial_n\opLog(f_{nn})(x))^2& \cr
\qquad\qquad= 2\lambda_n(x)B^{ij}(\partial_i\alpha)(x)(\partial_j\alpha)(x) - \frac{2}{n}(\partial_n\alpha)(x)^2.& \cr}$$
%
Thus
%
$$(\Cal{L}_f f_{nn})(x) \geq -C_1-C_1\lambda_n(x) - \frac{2}{n}(\partial_n\alpha)(x)^2 + 2\lambda_n(x)B^{ij}(x)(\partial_i\alpha)(x)(\partial_j\alpha)(x),
$$
%
and so, by Lemma \procref{DerivativeOfLogarithm},
%
$$
(\Cal{L}_f\alpha)(x) \geq -\frac{C_1}{\lambda_n(x)}-C_1-\frac{2}{n\lambda_n(x)}(\partial_n\alpha_n)(x)^2
 + B^{ij}(x)(\partial_i\alpha(x)(\partial_j\alpha(x)).
$$
%
Finally, by \eqnref{BasicEquation} and Lemma \procref{LowerBoundsOfTraceOfHessian},
%
$$
\lambda_n(x) \geq \frac{1}{n}\opTr(D^2f(x)) \geq F(D^2f(x)) = \phi(x)G(Df(x)) \geq \inf_{y\in\overline{\Omega}}\phi(y)>0,
$$
%
and the result follows.\qed
\medskip
The final term in Lemma \procref{ThirdBarrierFunction} makes this relation insufficient in itself for a direct application of the maximum principal. It is for this reason that the auxiliary function is required in the proof of the following theorem.
%
\proclaim{Theorem \nextprocno}
%
\noindent There exists $C>0$ which only depends on $\|\phi\|_2$, $\minf_{x\in\overline{\Omega}}\phi(x)$, $\delta(\hat{f})$, $\|\hat{f}\|_2$ and $\|f\|_1$ such that if $f\geq\hat{f}$ then,
%
$$
\|f\|_2 \leq C.
$$
%
\endproclaim
%
\proof For $A>0$, consider the function $\phi_A:\overline{\Omega}\rightarrow\Bbb{R}$ given by:
%
$$
\phi_A := \mu_n - A(f-\hat{f}).
$$
%
It suffices to prove that $\phi_A\leq C$ for some constants $A$ and $C$ which both depend only on $\|\phi\|_2$, $\minf_{x\in\overline{\Omega}}\phi(x)$, $\delta(\hat{f})$, $\|\hat{f}\|_2$ and $\|f\|_1$. However, by compactness of $\overline{\Omega}$, $\phi_A$ assumes its maximum at some point $x\in\overline{\Omega}$, say. First suppose that $x$ is a boundary point of $\Omega$. Let $C_1$ be as in Theorem \procref{SecondOrderBounds}. Observe that $C_1$ only depends on $\|\phi\|_1$, $\minf_{x\in\overline{\Omega}}\phi(x)$, $\delta(\hat{f})$, $\|f\|_2$ and $\|f\|_1$ and
%
$$
\phi_A(x) = \mu_n(x) = \opLog(\|D^2f(x)\|) \leq \opLog(C_1),
$$
%
as desired.
\par
Now suppose that $x$ is an interior point of $\Omega$. Let $C_2$ be as in Lemma \procref{ThirdBarrierFunction} and fix $A:=(C_2 + 1)\delta(\hat{f})^{-1}$. By Theorem \procref{SuperHarmonicFunctions},
%
$$
(\Cal{L}_f\phi_A)(x) \geq 1 - \frac{2}{n\lambda_n(x)}(\partial_n(\phi_A + A(f-\hat{f})))(x)^2,
$$
%
in the weak sense. Now let $\alpha:\Omega\rightarrow\Bbb{R}$ be such that $\alpha\leq\phi_A$ and $\alpha(x)=\phi_A(x)$. In particular, $\alpha$ attains its maximum at $x$, so that $(\partial_n\alpha)(x)=0$. Using the fact that $f-\hat{f}\geq 0$, this yields
%
$$\eqalign{
(\Cal{L}_f\alpha)(x) &\geq 1 - \frac{2A^2}{n\lambda_n(x)}(\partial_n(f-\hat{f}))(x)^2\cr
&\geq 1 - \frac{2A^2}{n}(\|f\|_1 + \|\hat{f}\|_1)e^{-\alpha(x)}.\cr}
$$
%
However, by the maximum principal,
%
$$
(\Cal{L}_f\alpha)(x) \leq 0,
$$
%
so that
%
$$
\phi_A(x) \leq \alpha(x) \leq \opLog\left(\frac{2A^2}{n}(\|f\|_1 + \|\hat{f}\|_1)\right),
$$
%
as desired. This completes the proof.\qed
%
\newsubhead{Higher order bounds}
%
Up to this point, we have obtained a-priori $C^2$ bounds for solutions of \eqnref{BasicEquation} satisfying $f\geq\hat{f}$. We review in this section the general principals required to obtain a-priori bounds of arbitrary order.
\subheadlabel{HigherOrderBounds}
\par
We first describe how a-priori $C^k$ bounds are obtained for all $k$ provided we have already obtained a-priori $C^{2+\alpha}$ bounds for some $\alpha>0$ (H\"older spaces and H\"older norms will be introduced and discussed in more detail in Section \subheadref{HolderSpaces}). Let $M$ be a compact manifold with boundary, let $U$ be an open subset of $\oplus_{i=0}^2\opSymm(i,\Bbb{R}^n)$ and let $\Phi:M\times\overline{\Omega}\times U\rightarrow\Bbb{R}$ be a smooth function. We consider the manifold $M$ as the parameter space for a smooth family of functions from $\overline{\Omega}\times U$ into $\Bbb{R}$. For all $\xi\in\oplus_{i=0}^1\opSymm(i,\Bbb{R}^n)$, we define $U_\xi\subseteq\opSymm(2,\Bbb{R}^n)$ by
%
$$
U_\xi := \left\{ A\in\opSymm(2,\Bbb{R}^n)\ |\ (\xi,A)\in U\right\},
$$
%
and for all $(p,x,\xi)\in M\times\overline{\Omega}\times\oplus_{i=0}^1\opSymm(i,\Bbb{R}^n)$, we define $\Phi_{p,x,\xi}:U_\xi\rightarrow\Bbb{R}$ by $\Phi_{x,p,\xi}(A) := \Phi(p,x,\xi,A)$. As in Section \subheadref{BasicPropertiesOfF}, for all $(p,x,\xi,A)\in M\times\overline{\Omega}\times U$, we identify $D\Phi_{p,x,\xi}(A)$ with an element of $\opSymm(2,\Bbb{R}^n)$. We say that $\Phi$ is \gloss{elliptic} whenever $D\Phi_{x,p,\xi}(A)$ is positive-definite for all $(p,x,\xi,A)\in M\times \overline{\Omega}\times U$. The following result encapsulates much of classical Schauder theory (c.f. Chapter $6$ of \cite{GilbTrud}).
%
\proclaim{Theorem \nextprocno}
%
\noindent If $\Phi$ is elliptic, then for every compact subset $K\subseteq U$, for every $\phi\in C^\infty(\partial\Omega)$, for all $B>0$, for all $\alpha\in]0,1[$ and for all $k\in\Bbb{N}$, there exists $C>0$ such that if $p$ is a point in $M$ and if $g:\overline{\Omega}\rightarrow\Bbb{R}$ is a smooth function with the properties that
\medskip
\myitem{(1)} $J^2(g)(x)\in K$ for all $x\in\overline{\Omega}$;
\medskip
\myitem{(2)} $\Phi(p,x,J^2g(x))=0$ for all $x\in\overline{\Omega}$;
\medskip
\myitem{(3)} $\|g\|_{2+\alpha}\leq B$; and
\medskip
\myitem{(4)} $g|_{\partial\Omega}=\phi$,
\medskip
\noindent then
%
$$
\|g\|_k\leq C.
$$
%
\endproclaim
\proclabel{Schauder}
%
We now show how a-priori $C^{2+\alpha}$ bounds are obtained from a-priori $C^2$ bounds. Let $M$ be a compact manifold with boundary, let $U$ be an open subset of $\oplus_{i=0}^1\opSymm(i,\Bbb{R}^n)$, let $\Gamma\subseteq\opSymm$ be the open cone of positive-definite, symmetric matrices, and let $\Phi:M\times\overline{\Omega}\times U\times\Gamma\rightarrow\Bbb{R}$ be a smooth function. As before, for all $(p,x,\xi)\in M \times\overline{\Omega}\times U$, we define $\Phi_{p,x,\xi}:\Gamma\rightarrow\Bbb{R}$ by $\Phi_{p,x,\xi}(A) := \Phi(p,x,\xi,A)$. The following result is a special case of Theorem $1$ of \cite{CaffNirSpruckII}.
%
\proclaim{Theorem \nextprocno}
%
\noindent Suppose that $\Phi$ is elliptic and that for all $(p,x,\xi)\in M\times\overline{\Omega}\times U$, $\Phi_{p,x,\xi}$ is concave. Then, for every compact $K\subseteq U$, for every $\phi\in C^\infty(\partial\Omega)$ and for all $B>0$, there exists $\alpha\in]0,1[$ and $C>0$ such that if $p$ is a point in $M$ and if $g:\overline{\Omega}\rightarrow\Bbb{R}$ is a smooth function with the properties that
\medskip
\myitem{(1)} $J^2g(x)\in K\times\Gamma$ for all $x\in\overline{\Omega}$;
\medskip
\myitem{(2)} $\Phi(p,x,J^2g(x))=0$ for all $x\in\overline{\Omega}$;
\medskip
\myitem{(3)} $\|g\|_2\leq B$; and
\medskip
\myitem{(4)} $g|_{\partial\Omega}=\phi$,
\medskip
\noindent then
%
$$
\|g\|_{2+\alpha}\leq C.
$$
%
\endproclaim
\proclabel{Krylov}
%
We now return to the case where
%
$$
\Phi(p,x,(t,\xi,A)) = F(A) - \phi(p,x) G(p,\xi),
$$
%
where $\phi>0$, $G\geq 1$ and $\xi\mapsto G(p,\xi)$ is concave for all $p$.
%
\proclaim{Theorem \nextprocno}
%
\noindent Let $(p_m)_\minn$ be a sequence of points in $M$ and let $(f_m)_\minn,(\hat{f}_m)_\minn\in C^\infty_0(\overline{\Omega})$ be strictly convex functions such that for all $m$, $f_m\geq\hat{f}_m$ and, for all $x\in\overline{\Omega}$,
%
$$
\Phi(p_m,x,J^2\hat{f}_m) \geq 0 = \Phi(p_m,x,J^2 f_m).
$$
%
\noindent If there exists $x_0\in M$ towards which $(x_m)_\minn$ converges and $\hat{f}_\infty\in C^\infty_0(\overline{\Omega})$ towards which $(\hat{f}_m)_\minn$ converges in the $C^\infty$ sense, then there exists $f_\infty\in C^\infty_0(\overline{\Omega})$ towards which $(f_m)_\minn$ subconverges in the $C^\infty$ sense.
%
\endproclaim
\proclabel{Compactness}
%
\proof By Lemma \procref{ZeroethAndFirstOrderBounds}, there exists $C_1>0$ such that for all $m$, $\|f_m\|_1 \leq C_1$. By Theorem \procref{SecondOrderBounds}, there exists $C_2>0$ such that, for all $m$, $\|f_m\|_2\leq C_2$. By Corollary \procref{ConcavityOfF}, $\Phi_{(p,x,(t,\xi))}$ is concave for all $(p,x,(t,\xi))$. Thus, by Theorem \procref{Krylov}, there exists $\alpha>0$ and $C_{2+\alpha}>0$ such that, for all $m$, $\|f_m\|_{2+\alpha} \leq C_{2+\alpha}$. By Theorem \procref{Schauder}, for all $k\in\Bbb{N}$, there exists $C_k>0$ such that, for all $m$, $\|f_m\|_k \leq C_k$. It now follows by the Arzela-Ascoli theorem (c.f. Theorem $11.28$ of \cite{Rudin}) that there exists $f_\infty\in C^\infty_0(\overline{\Omega})$ towards which $(f_m)_\minn$ subconverges, and this completes the proof.\qed 

==> glossary.tex <==
shape operator\hskip 1em\relax 1\par 
Weingarten operator\hskip 1em\relax 1\par 
gaussian curvature\hskip 1em\relax 2\par 
extrinsic curvature\hskip 1em\relax 2\par 
strictly convex\hskip 1em\relax 2\par 
outer barrier\hskip 1em\relax 3\par 
lower barrier\hskip 1em\relax 8\par 
elliptic\hskip 1em\relax 24\par 
differentiable\hskip 1em\relax 28\par 
derivative\hskip 1em\relax 28\par 
smooth\hskip 1em\relax 28\par 
Banach space\hskip 1em\relax 29\par 
submanifold\hskip 1em\relax 29\par 
trivialising chart\hskip 1em\relax 29\par 
Fredholm\hskip 1em\relax 30\par 
index\hskip 1em\relax 30\par 
Fredholm\hskip 1em\relax 30\par 
solution space\hskip 1em\relax 30\par 
H\"older semi-norm\hskip 1em\relax 31\par 
H\"older norm\hskip 1em\relax 32\par 
elliptic function\hskip 1em\relax 34\par 
solution space\hskip 1em\relax 36\par 
Hausdorff distance\hskip 1em\relax 39\par 
supporting normal\hskip 1em\relax 41\par 
graph\hskip 1em\relax 44\par 
convex hull\hskip 1em\relax 47\par 
local geodesic property\hskip 1em\relax 48\par 
strictly contained in a hemisphere\hskip 1em\relax 50\par 
open half-space\hskip 1em\relax 59\par 
non-antipodal\hskip 1em\relax 61\par 
great-circular arc\hskip 1em\relax 61\par 
convex\hskip 1em\relax 61\par 
open hemisphere\hskip 1em\relax 61\par 
southern hemisphere\hskip 1em\relax 61\par 
affine projection\hskip 1em\relax 61\par 
dual\hskip 1em\relax 63\par 
link\hskip 1em\relax 66\par 
link\hskip 1em\relax 66\par 
normal\hskip 1em\relax 74\par 
shape operator\hskip 1em\relax 74\par 
strong barrier\hskip 1em\relax 89\par 
weak barrier\hskip 1em\relax 89\par 
volume\hskip 1em\relax 94\par 
regular\hskip 1em\relax 97\par 
singular set\hskip 1em\relax 97\par 

